Finite-time stabilization via impulse control of degenerate singular parabolic equations

This paper examines the impulse controllability of degenerate singular parabolic equations through a modern framework focused on finite-time stabilization. Furthermore, we provide an explicit estimate for the exponential decay of the solution. The proof of our main result combines a logarithmic convexity estimate with specific spectral properties. Finally, we establish the existence and uniqueness of the minimal norm impulse control associated with the system.

==> References.tex <==
\begin{thebibliography}{9}

\bibitem{BAJS}
    \newblock B. Allal and J. Salhi, 
    \newblock Pointwise Controllability for Degenerate Parabolic Equations by the Moment Method,
    \newblock \emph{J. Dyn. Control Syst.}, \textbf{26} (2020), 349--362.

\bibitem{ACM'21}
    \newblock E. M. Ait Ben Hassi, S. E. Chorfi and L. Maniar,
    \newblock An inverse problem of radiative potentials and initial temperatures in parabolic equations with dynamic boundary conditions,
    \newblock \emph{J. Inverse Ill-Posed Probl.}, \textbf{30} (2022), 363--378. 

\bibitem{ACM'21'}
    \newblock E. M. Ait Ben Hassi, S. E. Chorfi and L. Maniar,
    \newblock Identification of source terms in heat equation with dynamic boundary conditions,
    \newblock \emph{Math. Meth. Appl. Sci.}, \textbf{45} (2022), 2364--2379.
    
\bibitem{ACM'21''}
    \newblock E. M. Ait Ben Hassi, S. E. Chorfi and L. Maniar,
    \newblock Inverse problems for general parabolic systems and application to Ornstein-Uhlenbeck equation, \, arXiv: 2110.01321 (2022).    
    
\bibitem{ACMO'20}
     \newblock E. M. Ait Ben Hassi, S. E. Chorfi, L. Maniar and O. Oukdach,
     \newblock Lipschitz stability for an inverse source problem in anisotropic parabolic equations with dynamic boundary conditions,
     \newblock \emph{Evol. Equat. and Cont. Theo.}, \textbf{10} (2021), 837--859.

    
\bibitem{ABWZ}
     \newblock A. Ben Aissa and W. Zouhair,
     \newblock Qualitative properties for the $1-D$ impulsive wave equation: controllability and observability,
     \newblock \emph{Quaestiones Mathematicae}, (2021), doi: \burl{https://doi.org/10.2989/16073606.2021.1940346}{10.2989/16073606.2021.1940346}.
     

\bibitem{BCMO'20}
     \newblock I. Boutaayamou, S. E. Chorfi, L. Maniar and O. Oukdach,
     \newblock The cost of approximate controllability of heat equation with general dynamical boundary conditions, \emph{Portugal. Math.}, \textbf{78} (2021), 65--99.

\bibitem{BP'18} 
    \newblock R. Buffe and K. D. Phung,
    \newblock A spectral inequality for degenerate operators and applications,
    \newblock \emph{C. R. Math. Acad. Sci. Paris}, \textbf{356} (11-12) (2018) 1131--1155.

\bibitem{RBKDP} 
    \newblock R. Buffe and K. D. Phung,
    \newblock Observation estimate for the heat equations with Neumann boundary condition via logarithmic convexity,
    \newblock preprint (2021), \burl{https://arxiv.org/abs/2105.12977}{arXiv:2105.12977}
     
\bibitem{CGMZ'22}
    \newblock S. E. Chorfi, G. El. Guermai,  L. Maniar, and W. Zouhair,
    \newblock Impulsive  null approximate controllability for heat equation with dynamic boundary conditions,
    \newblock \emph{Math. Control Rel. Fields}, (2022), doi: \burl{https://dx.doi.org/10.3934/mcrf.2022026}{10.3934/mcrf.2022026}.
    
\bibitem{CGMZ'221}
    \newblock S. E. Chorfi, G. El. Guermai,  L. Maniar, and W. Zouhair,
    \newblock Logarithmic convexity and impulsive controllability for the one-dimensional heat equation with dynamic boundary conditions,
    \newblock \emph{IMA J. Math. Control. Inf.}, (2022), doi: \burl{https://academic.oup.com/imamci/advance-article-abstract/doi/10.1093/imamci/dnac013/6599076?redirectedFrom=fulltext&login=false}{10.1093/imamci/dnac013}.
    
\bibitem{SEEGLMWZ22}
    \newblock S. E. Chorfi, G. El. Guermai,  L. Maniar, and W. Zouhair,
    \newblock Identification of source terms in wave equation with dynamic boundary conditions,
    \newblock \emph{Math. Methods Appl. Sci. }, (2022), doi: \burl{https://onlinelibrary.wiley.com/doi/10.1002/mma.8556}{10.1002/mma.8556}.

\bibitem{Coron2017}
    \newblock J. M. Coron, and H. M. Nguyen,
    \newblock  Null controllability and finite time stabilization for the heat equations with variable coefficients in space in one dimension via backstepping approach,
    \newblock \emph{Arch Ration Mech Anal.}, \textbf{225} (2017), 993--1023.

\bibitem{FH'11}
    \newblock Z. J. Z. Farkas and P. Hinow,
    \newblock Physiologically structured populations with diffusion and dynamic boundary conditions,
    \newblock \emph{Math. Biosci. Eng.}, \textbf{8} (2011), 503--513.
    
\bibitem{Ci'16}
	       \newblock C. G. Gal, 
	       \newblock The Role of Surface Diffusion in Dynamic Boundary Condition: Where Do we Stand, \newblock \emph{Milan J. Math.}, \textbf{83},  (2015), 237--278. 
        
\bibitem{CGHL18}
	       \newblock C. Guevara and H. Leiva,
	       \newblock Controllability of the impulsive semilinear heat equation with memory and delay,
	       \newblock \emph{J. Dyn. Control Syst.},\textbf{24} (2018), 1--11.

\bibitem{Go'06}
    \newblock G. R. Goldstein,
    \newblock Derivation and physical interpretation of general boundary conditions,
    \newblock \emph{Adv. Diff. Equ.}, \textbf{11} (2006), 457--480.
    
\bibitem{Jose}
    \newblock  S.A. Jose, W. Yukunthorn, J. E. N. Valdes and H. Leiva,
    \newblock Some existence, uniqueness and stability results of nonlocal random impulsive integro-differential equations,
    \newblock \emph{Appl. Math. - Notes}, \textbf{20} (2020),481--492.

\bibitem{ka}
    \newblock A. Y. Khapalov,
    \newblock Exact controllability of second-order hyperbolic equations with impulse controls,
    \newblock \emph{Applicable Analysis}, \textbf{63} (1996), 223--238.
    
\bibitem{KM'19}
   \newblock A. Khoutaibi and L. Maniar,
   \newblock Null controllability for a heat equation with dynamic boundary conditions and drift terms,
   \newblock \emph{Evol. Equat. and Cont. Theo.}, \textbf{9} (2020), 535--559.
   
\bibitem{La'32}
    \newblock R. E. Langer,
    \newblock A problem in diffusion or in the flow of heat for a solid in contact with a fluid,
    \newblock \emph{Tohoku Math. J.}, \textbf{35} (1932), 260--275.
    
\bibitem{SLAPWZ2}
    \newblock S. Lalvay, A. Padilla-Segarra, and W. Zouhair,
    \newblock On the existence and uniqueness of solutions for non-autonomous semi-linear systems with non-instantaneous impulses, delay, and non-local conditions,
    \newblock \emph{Miskolc Math. Notes,} Vol. \textbf{23} (2022), 295--310.

\bibitem{McKenna}
    \newblock H. Leiva and W. Zouhair,
    \newblock Controllability of suspension bridge model proposed by Lazer and McKenna under the influence of impulses, delays, and non-local conditions,
    \newblock \emph{ Dyn. Contin. Discrete Impuls. Syst.,}  \textbf{30} (2023), 123-133.

    
\bibitem{LHWZME2}
    \newblock H. Leiva, W. Zouhair and D. Cabada,
    \newblock Existence, uniqueness, and controllability analysis of Benjamin-Bona-Mahony equation with non-instantaneous impulses, delay, and non-local conditions,
    \newblock \emph{J. Math. Control Sci.,}  \textbf{07} (2021), 91-108.

\bibitem{Zouhair2022'} 
    \newblock H. Leiva, W. Zouhair, M. E. Entekhabi, and E. Lucena,
    \newblock Approximate controllability of semi-linear heat equation with Non-instantaneous impulses, memory and delay,
    \newblock preprint (2022), \burl{
https://doi.org/10.48550/arXiv.2008.02094}{arXiv.2008.02094}

\bibitem{MMOS'23}
    \newblock H.Maarouf, L.Maniar, I.Ouelddris and J.Salhi,
    \newblock \emph{Impulse controllability for degenerate singular parabolic equations via logarithmic convexity method},
    \newblock \emph{IMA J. of Math. Control and Info.}, \textbf{40} (4). (2023). 593–617. \href{https://doi.org/10.1093/imamci/dnad025}{https://doi.org/10.1093/imamci/dnad025}.

\bibitem{MMS'17}
    \newblock L. Maniar, M. Meyries and R. Schnaubelt,
    \newblock Null controllability for parabolic equations with dynamic boundary conditions of reactive-diffusive type,
    \newblock \emph{Evol. Equat. and Cont. Theo.}, \textbf{6} (2017), 381--407.

\bibitem{MOZ2022}
    \newblock L. Maniar, O. Oukdach and W. Zouhair,
    \newblock Lebeau-Robbiano
     inequality for heat equation with dynamic boundary conditions and optimal null controllability,
    \newblock \emph{Differ. Equ. Dyn. Syst.},(2022), To appear.

\bibitem {MBEYR}
   \newblock B. Miller and E. Y. Rubinovich,
   \newblock \emph{Impulsive Control in Continuous and Discrete-Continuous Systems},
   \newblock Springer Science and Business Media, \textbf{6}, 2003.  
   
\bibitem{pkm}
    \newblock K. D. Phung,
    \newblock Carleman commutator approach in logarithmic convexity for parabolic equations,
    \newblock \emph{Math. Control Rel. Fields}, \textbf{8} (2018), 899--933.


\bibitem{Sa'20}
    \newblock N. Sauer,
    \newblock Dynamic boundary conditions and the Carslaw-Jaeger constitutive relation in heat transfer,
    \newblock \emph{SN Partial Differ. Equ. Appl.}, \textbf{1} (2020), 1--20.
 
\bibitem{DSMSM21}
    \newblock D. Sadali and  M. S. Moulay,
    \newblock A New Carleman Inequality for a Heat Equation in Presence of Singularities and Controllability Consequences,
    \newblock \emph{J. Dyn. Control Syst.}, \textbf{27} (2021), 51--65.
 
\bibitem {YT}
   \newblock Y. Tao,
   \newblock \emph{Impulsive Control Theory}, 
   \newblock Springer, Science and Business Media, \textbf{272}, 2001.
   
\bibitem {VTMN} 
    \newblock T. M. N. Vo, 
    \newblock The local backward heat problem,
    \newblock preprint (2017),
  \burl{https://arxiv.org/abs/1704.05314}{arXiv:1704.05314}.  

\end{thebibliography}


